VLG-Net: Video-Language Graph Matching Network for Video Grounding

Grounding language queries in videos aims at identifying the time interval (or moment) semantically relevant to a language query. The solution to this challenging task demands understanding videos' and queries' semantic content and the fine-grained reasoning about their multi-modal interactions. Our key idea is to recast this challenge into an algorithmic graph matching problem. Fueled by recent advances in Graph Neural Networks, we propose to leverage Graph Convolutional Networks to model video and textual information as well as their semantic alignment. To enable the mutual exchange of information across the modalities, we design a novel Video-Language Graph Matching Network (VLG-Net) to match video and query graphs. Core ingredients include representation graphs built atop video snippets and query tokens separately and used to model intra-modality relationships. A Graph Matching layer is adopted for cross-modal context modeling and multi-modal fusion. Finally, moment candidates are created using masked moment attention pooling by fusing the moment's enriched snippet features. We demonstrate superior performance over state-of-the-art grounding methods on three widely used datasets for temporal localization of moments in videos with language queries: ActivityNet-Captions, TACoS, and DiDeMo.

==> sections/symbols.tex <==
Video $V$
Language $L$
ground-truth moment $(\tau_s, \tau_e)$
candidate predictions $m$ 
the start time $t_{s,k}$
end time $t_{e,k}$
confidence score $p_k$
video representations $X_v$
language representations $X_l$
feature dimension of each snippet vector $c_v$
number of snippets $n_v$



==> tables/table_ablation1.tex <==
\centering % centering table
\resizebox{0.97\linewidth}{!}{%
\scalebox{1.0}{
\begin{tabular}{l|ccc|c} % creating seven columns

\toprule
 
\multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{Modules} & \multirow{2}{*}{R@1 IoU0.7} \\ %in %& R@1 \\& IoU0.7
& GCNeXt. & SyntacGCN. & Graph Matching \\ 
\midrule
                                & \cmark & \cmark & \cmark &  $\mathbf{29.42}$ \\ 
ActivityNet-                    & \xmark & \cmark & \cmark &  $28.16$          \\
Captions                        & \cmark & \xmark & \cmark &  $28.41$          \\
                                & \cmark & \cmark & \xmark &  $14.34$          \\

\midrule
\multirow{4}{*}{TACoS}  & \cmark & \cmark & \cmark &  $\mathbf{31.39}$ \\
                        & \xmark & \cmark & \cmark &  $29.87$          \\
                        & \cmark & \xmark & \cmark &  $30.49$          \\
                        & \cmark & \cmark & \xmark &  $7.42$           \\
\bottomrule
\end{tabular}
}
}
% \vspace{.1cm}
\caption{\label{tab:ablation1}{\bf Ablation of main modules.} We report the performance of our architecture when specific modules are removed, as well as our best performance for ActivityNet-Captions and TACoS datasets. \SQ{remember the last column is wrong}} 


==> tables/table_charades.tex <==

\centering % centering table
%\resizebox{\linewidth}{!}{%
\scalebox{1.0}{
\begin{tabular}{l|cc|cc} % creating seven columns
\toprule
&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
&   R@1 & R@5 & R@1 & R@5 \\ 
\midrule
Single positive    & XX & XX & XX &	XX \\
Multiple positives & XX & XX & XX &	XX \\
\bottomrule
\end{tabular}
}
%}
% \vspace{.1cm}
\caption{\label{tab:single_video_performance} 
{\bf Title table:Brief description.}}



\centering % centering table
%\resizebox{\linewidth}{!}{%
\scalebox{1.0}{
\begin{tabular}{l|cccc} % creating seven columns
\toprule
&   K=1 & K=10 & K=100 & MR \\ 
\midrule
Single positive    & XX & XX & XX &	XX \\
Multiple positives & XX & XX & XX &	XX \\
\bottomrule
\end{tabular}
}
\caption{\label{tab:charades} 
{\bf Title table:Brief description.}}


==> tables/table_overfit.tex <==

\centering % centering table
\resizebox{0.8\linewidth}{!}{%
% \scalebox{1.0}{
\begin{tabular}{l|cc|cc} % creating seven columns
\toprule
&   \multicolumn{2}{c|}{R@1  }& \multicolumn{2}{c}{R@5  } \\ 
&   IoU=0.5 & IoU=0.5 & IoU=0.5 & IoU=0.5 \\ 
\midrule
LGI~\cite{Mun_2020_CVPR}      & $99.85$ & $99.06$ & -- &	-- \\
2D-TAN~\cite{2DTAN_2020_AAAI} & XX & XX & XX &	XX \\
DRN~\cite{Zeng_2020_CVPR}     & XX & XX & XX &	XX \\
\bottomrule
\end{tabular}
}
%}
% \vspace{.1cm}
\caption{\label{tab:overfit} 
{\bf Evaluation on training set. }  We evaluate recently published methods on the training set to determine how relevant is the overfitting issue. 
}




==> tables/table_rebuttal.tex <==
\vspace{-0.7cm}
\centering % centering table
{\setlength{\tabcolsep}{7pt}
% \renewcommand{\arraystretch}{1} 
\resizebox{\linewidth}{!}{%
\scalebox{1.0}{
\begin{tabular}{l|cc|cc} % creating seven columns
\toprule
ActivityNet &   \multicolumn{2}{c|}{~~~~~~~~~~~~~~~~R@1~~~~~~~~~~~~~~~~~  } & \multicolumn{2}{c}{~~~~~~~~~~~~~~~~R@5~~~~~~~~~~~~~~~~~~  }   \\ 
Captions&   ~~~~~IoU0.5  & IoU0.7  & ~~~~~IoU0.5  & IoU0.7  \\ 
\midrule
CSMGAN~~  & ~~~~~$\mathbf{49.11}$ &          $29.15$ & ~~~~~$\mathbf{77.43}$ & $59.63$  \\
VLG-Net &         ~~~~~$46.32$  & $\mathbf{29.82}$ &  ~~~~~$        77.15$  & $\mathbf{63.33}$ \\
\end{tabular}
}}}

\centering % centering table
\resizebox{\linewidth}{!}{%
\scalebox{1.0}{
\begin{tabular}{l|ccc|ccc} % creating seven columns
\toprule
\multirow{2}{*}{TACoS} &   \multicolumn{3}{c|}{R@1  }& \multicolumn{3}{c}{R@5  }   \\ 
&  IoU0.1 & IoU0.3  & IoU0.5  & IoU0.1  & IoU0.3  & IoU0.5  \\ 
\midrule
CSMGAN~~~ & $42.74$ & $33.90$ & $27.09$ & $68.97$ & $53.98$ & $41.22$  \\
VLG-Net   &  $\mathbf{57.21}$ & $\mathbf{45.46}$ & $\mathbf{34.19}$ & $\mathbf{81.80}$ & $\mathbf{70.38}$ & $\mathbf{56.56}$ \\
% \bottomrule
\end{tabular}
}
}

\centering % centering table
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1} 
\resizebox{\linewidth}{!}{%
\scalebox{1.0}{
\begin{tabular}{l|ccc|ccc} % creating seven columns
\toprule
\multirow{2}{*}{DiDeMo} &   \multicolumn{3}{c|}{R@1  }& \multicolumn{3}{c}{R@5  }   \\ 
&  IoU0.5 & IoU0.7  & IoU1.0  & IoU0.5  & IoU0.7  & IoU1.0  \\ 
\midrule
\textcolor{mygray}{MAN\textsubscript{(VGG16)}} & \textcolor{mygray}{$\mathbf{41.24}$} & \textcolor{mygray}{$\underline{20.54}$} & \textcolor{mygray}{$-$} & \textcolor{mygray}{$\underline{83.21}$} & \textcolor{mygray}{$\underline{51.85}$} & \textcolor{mygray}{$-$}  \\
CSMGAN  & $29.44$ & $19.16$ & $-$ & $70.77$ & $41.61$ & $-$  \\
VLG-Net & $\underline{33.35}$ & $\mathbf{25.57}$ & $\mathbf{25.57}$ & $\mathbf{88.86}$ & $\mathbf{71.72}$ & $\mathbf{71.65}$ \\
\bottomrule
\end{tabular}
}
}
% \vspace{-.02cm}
\caption{\label{tab:reuttal}{Additional performance comparison for ActivityNet-Captions (top), TACoS (center) and DiDeMo (bottom).}  
}










==> tables/table_rebuttal2.tex <==
\vspace{-0.8cm}
\centering % centering table
{\setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1} 
\resizebox{\linewidth}{!}{%
\scalebox{1.0}{
\begin{tabular}{ll|cc|cc} % creating seven columns
\toprule
\hspace{-0.1cm}\parbox[t]{0mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Activitynet}}}& &   \multicolumn{2}{c|}{~~~~~~~~~~~~~~~~~~~R@1~~~~~~~~~~~~~~~~~~~} & \multicolumn{2}{c}{~~~~~~~~~~~~~~~~~~~R@5~~~~~~~~~~~~~~~~~~~~}   \\ 
& &   ~~~~~~IoU0.5  & IoU0.7  & ~~~~~~IoU0.5  & IoU0.7  \\ \cline{3-6}
 & \hspace{-0.25cm} \cite{liu2020jointly}  & ~~~~~~$\mathbf{49.11}$ &          $29.15$ & ~~~~~~$\mathbf{77.43}$ & $59.63$  \\
& \hspace{-0.25cm} VLG \hspace{0.075cm} &         ~~~~~~$46.32$  & $\mathbf{29.82}$ &  ~~~~~~ $77.15$  & $\mathbf{63.33}$ \\
\end{tabular}
}}}

\centering % centering table
\resizebox{\linewidth}{!}{%
\scalebox{1.0}{
\begin{tabular}{ll|ccc|ccc} % creating seven columns
\toprule
\parbox[t]{0mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{TACoS}}}
& &  IoU0.1 & IoU0.3  & IoU0.5  & IoU0.1  & IoU0.3  & IoU0.5  \\ \cline{3-8}
&\cite{liu2020jointly}~~~~~ & $42.74$ & $33.90$ & $27.09$ & $68.97$ & $53.98$ & $41.22$  \\
& VLG \hspace{0.075cm}   &  $\mathbf{57.21}$ & $\mathbf{45.46}$ & $\mathbf{34.19}$ & $\mathbf{81.80}$ & $\mathbf{70.38}$ & $\mathbf{56.56}$ \\
% \bottomrule
\end{tabular}
}
}

\centering % centering table
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1} 
\resizebox{\linewidth}{!}{%
\scalebox{1.0}{
\begin{tabular}{ll|ccc|ccc} % creating seven columns
\toprule
\parbox[t]{0mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{DiDeMo}}}
& &  IoU0.5 & IoU0.7  & IoU1.0  & IoU0.5  & IoU0.7  & IoU1.0  \\ 
\cline{3-8}
&\textcolor{mygray}{[78]} & \textcolor{mygray}{$\mathbf{41.24}$} & \textcolor{mygray}{$\underline{20.54}$} & \textcolor{mygray}{$-$} & \textcolor{mygray}{$\underline{83.21}$} & \textcolor{mygray}{$\underline{51.85}$} & \textcolor{mygray}{$-$}  \\
& \cite{liu2020jointly}  & $29.44$ & $19.16$ & $-$ & $70.77$ & $41.61$ & $-$  \\
&VLG \hspace{0.075cm} & $\underline{33.35}$ & $\mathbf{25.57}$ & $\mathbf{25.57}$ & $\mathbf{88.86}$ & $\mathbf{71.72}$ & $\mathbf{71.65}$ \\
\bottomrule
\end{tabular}
}
}
\caption{\label{tab:reuttal}{Additional performance comparison for ActivityNet-Captions (top), TACoS (center) and DiDeMo (bottom).}  
}









